SaccadeCam: Adaptive Visual Attention for Monocular Depth Sensing

Most monocular depth sensing methods use conventionally captured images that are created without considering scene content. In contrast, animal eyes have fast mechanical motions, called saccades, that control how the scene is imaged by the fovea, where resolution is highest. In this paper, we present the SaccadeCam framework for adaptively distributing resolution onto regions of interest in the scene. Our algorithm for adaptive resolution is a self-supervised network and we demonstrate results for end-to-end learning for monocular depth estimation. We also show preliminary results with a real SaccadeCam hardware prototype.

==> ablation/ablation1.tex <==


% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{3}{|c|}{\cellcolor[HTML]{FFCCC9}\textbf{Resolution (px/mm)}} & \multicolumn{19}{c|}{\cellcolor[HTML]{FFCE93}\textbf{Errors (RMSE)}} \\ \hline
% \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCE93} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFC9E}\textbf{Defocused}} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFC9E}\textbf{WAC}} & \multicolumn{2}{c|}{\cellcolor[HTML]{9AFF99}\textbf{\begin{tabular}[c]{@{}c@{}}Oracle 0\\ (foveate focused depth)\end{tabular}}} & \cellcolor[HTML]{DAE8FC}\textbf{\begin{tabular}[c]{@{}c@{}}Oracle 2\\ (No weighting)\\ black magic finetuned\end{tabular}} & \cellcolor[HTML]{DAE8FC}\textbf{\begin{tabular}[c]{@{}c@{}}Oracle 2\\ (.75/.25 Weighting)\\ black magic finetuned\end{tabular}} & \cellcolor[HTML]{DAE8FC}\textbf{\begin{tabular}[c]{@{}c@{}}Oracle 2\\ max(WAC, FOCUSED) \\ attention -- from scratch\end{tabular}} & \cellcolor[HTML]{DAE8FC}\textbf{\begin{tabular}[c]{@{}c@{}}Oracle 2\\ max(WAC, FOCUSED) \\ attention -- finetuned\end{tabular}} & \cellcolor[HTML]{9AFF99}\textbf{OURS} & \cellcolor[HTML]{9AFF99}\textbf{} & \cellcolor[HTML]{9AFF99}\textbf{} & \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Edges}} & \cellcolor[HTML]{DAE8FC}\textbf{Random} & \cellcolor[HTML]{DAE8FC}\textbf{} & \cellcolor[HTML]{DAE8FC}\textbf{} \\ \cline{5-22} 
% \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Focused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Defocused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{WAC}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCE93}\textbf{Focused}} & \cellcolor[HTML]{FFFC9E}\textbf{20 epochs} & \cellcolor[HTML]{FFFC9E}\textbf{Finetune} & \cellcolor[HTML]{FFFC9E}\textbf{20 epochs} & \cellcolor[HTML]{FFFC9E}\textbf{Finetune} & \cellcolor[HTML]{9AFF99}\textbf{20 epochs} & \cellcolor[HTML]{9AFF99}\textbf{Finetune} & \cellcolor[HTML]{DAE8FC}\textbf{RMSE} & \cellcolor[HTML]{DAE8FC}\textbf{RMSE} & \cellcolor[HTML]{DAE8FC} & \cellcolor[HTML]{DAE8FC} & \cellcolor[HTML]{9AFF99}\textbf{RMSE} & \cellcolor[HTML]{9AFF99}\textbf{\begin{tabular}[c]{@{}c@{}}Bandwidth \% \\ Correct\end{tabular}} & \cellcolor[HTML]{9AFF99}\textbf{Overlap \%} & \cellcolor[HTML]{DAE8FC}\textbf{RMSE} & \multicolumn{1}{l|}{\cellcolor[HTML]{DAE8FC}\textbf{Overlap \%}} & \cellcolor[HTML]{DAE8FC}\textbf{1} & \cellcolor[HTML]{DAE8FC}\textbf{3} & \cellcolor[HTML]{DAE8FC}\textbf{5} \\ \hline
% 70 & 31.30 & 27.11 & 4.960 & 5.188 & 5.089 & 5.238 & 5.136 & 4.850 & 4.837 & \textbf{5.058} & 5.130 (OURS = 5.123) & 5.184 & 5.135 & \textbf{5.058} & 99.1 & 95.6 & 5.109 & 12.7 & 5.102 & 5.124 & 5.094 \\ \hline
% 70 & 31.30 & 22.14 & 4.960 & 5.188 & 5.089 & 5.275 & 5.180 & 4.846 & 4.835 & 5.099 &  & 5.313 & 5.191 & \textbf{5.082} & 88.2 & 96.2 & 5.205 & 17.5 & 5.119 & 5.127 & 5.125 \\ \hline
% 70 & 31.30 & 15.65 & 4.960 & 5.188 & 5.089 & 5.507 & 5.311 & 4.848 & 4.842 & 5.183 &  & 5.536 & 5.298 & 5.107 & 94.3 & 97.25 & 5.428 & 26.3 & 5.226 & 5.267 & 5.189 \\ \hline
% 70 & 7.82 & 6.78 & 4.960 & 7.378 & 6.454 & 8.317 & 6.688 & 7.308 & 6.033 & 6.625 & \textbf{6.374 (OURS = 6.415)} &  &  & 6.612 & 98.8 & 91.4 & 6.668 & 2.6 & 6.502 & 6.486 & 6.416 \\ \hline
% 70 & 7.82 & 5.53 & 4.960 & 7.378 & 6.454 & 9.382 & 7.155 & 7.341 & 5.950 & 7.048 &  &  &  & 6.889 & 84.8 & 93.2 & \multicolumn{1}{l|}{7.066} & 4.9 & 6.636 & 6.613 & 6.623 \\ \hline
% 70 & 7.82 & 3.90 & 4.960 & 7.378 & 6.454 & 11.875 & 7.786 & 8.327 & 6.015 & 7.435 &  &  &  & 7.511 & 98.5 & 95.7 & \multicolumn{1}{l|}{7.711} & 6.6 & 7.049 & 7.033 & 6.908 \\ \hline
% \end{tabular}}
% \caption{}
% \label{tab:abl1}

% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|l|}
% \hline
% \rowcolor[HTML]{ECF4FF} 
% \multicolumn{3}{|c|}{\cellcolor[HTML]{FFCCC9}\textbf{Resolution (px/mm)}} & \multicolumn{6}{c|}{\cellcolor[HTML]{ECF4FF}\textbf{Errors (RMSE)}} \\ \hline
% \rowcolor[HTML]{ECF4FF} 
% \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{ECF4FF} & \cellcolor[HTML]{ECF4FF} & \cellcolor[HTML]{ECF4FF} & \multicolumn{2}{c|}{\cellcolor[HTML]{ECF4FF}\textbf{\begin{tabular}[c]{@{}c@{}}OURS\\ 1x bandwith\\ varying fovea resolution\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}} \\ \cline{7-8}
% \rowcolor[HTML]{ECF4FF} 
% \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Focused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Defocused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{WAC}} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}\textbf{Focused}} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}\textbf{Defocused}} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}\textbf{WAC}} & \textbf{\begin{tabular}[c]{@{}c@{}}varying fovea \\ ang. resolution\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}constant fovea \\ ang. resolution\end{tabular}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{CBCEFB}\textbf{Edges}}} \\ \hline
% 70 & 31.30 & 27.11 & 4.960 & 5.188 & 5.238 & \textbf{5.111} & 5.156 & 5.442 \\ \hline
% 70 & 31.30 & 22.14 & 4.960 & 5.188 & 5.275 & 5.281 & 5.240 & 5.539 \\ \hline
% % 70 & 31.30 & 15.65 & 4.960 & \textbf{5.188} & 5.507 &  &  & 5.770 \\ \hline
% 70 & 7.82 & 6.78 & 4.960 & 7.378 & 8.317 & 6.815 & \textbf{6.777} & 6.836 \\ \hline
% 70 & 7.82 & 5.53 & 4.960 & 7.378 & 9.382 &  & \textbf{7.181} & 7.422 \\ \hline
% % 70 & 7.82 & 3.90 & 4.960 & \textbf{7.378} & 11.875 &  &  & 8.761 \\ \hline
% \end{tabular}}
% \caption{}
% \label{tab:abl1}

% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{ECF4FF} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFCCC9}Bandwidth (px/mm)} & \multicolumn{7}{c|}{\cellcolor[HTML]{ECF4FF}Errors (RMSE)} \\ \hline
\rowcolor[HTML]{ECF4FF} 
\cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{ECF4FF} & \cellcolor[HTML]{ECF4FF} & \cellcolor[HTML]{ECF4FF} & \multicolumn{2}{c|}{\cellcolor[HTML]{ECF4FF}\textbf{OURS}} & \multicolumn{2}{c|}{\cellcolor[HTML]{ECF4FF}Color Edges} \\ \cline{7-10} 
\rowcolor[HTML]{ECF4FF} 
\multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}Full Res.} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}Target Res} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}WAC} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}Full Res.} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}Target Res.} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}WAC} & \textbf{No weighting} & \textbf{Fovea weighted more} & No weighting & Edges weighted more \\ \hline
70 & 35.0 & 30.31 & 4.960 & 5.144 & 5.202 & 5.087  & \textbf{5.053 } & 5.278 & 5.267 \\ \hline
70 & 31.30 & 27.11 & 4.960 & 5.188 & 5.238 & \textbf{5.111 } & 5.154  & 5.442 & 5.502 \\ \hline
70 & 27.11 & 23.48 & 4.960 & 5.209 & 5.264 & 5.173 & \textbf{5.151 } & 5.721 & 5.660 \\ \hline
70 & 7.82 & 6.78 & 4.960 & 7.378 & 8.317 & 6.815 & \textbf{6.552 } & 6.836 & 6.589 \\ \hline
70 & 7.82 & 5.53 & 4.960 & 7.378 & 9.382 & \textbf{7.106} & 7.132 & 7.422 & 7.157 \\ \hline
\end{tabular}}
\caption{SaccadeCam compared against equiangular (conventional) images. For a variety of bandwidth ratios of full resolution vs. target resolution, we show how the SaccadeCam framework (shown in Fig. \ref{fig:method}) outperforms images with conventionally uniformly distributed resolution across the FOV. While rendering the SaccadeCam method, we show how weighting the fovea in the A-B reconstruction in Fig. \ref{fig:method} can be advantageous. For edges, we use the same depth network as our results, but use a Canny edge detector as the attention mask instead of our learned attention mask. Notice how, at very low resolutions, the edge comparison is closer to our method. We assume this is because the resolution is so low in WAC that any fovea helps. However, in higher resolutions, the resolution must be more intelligently placed to boost the depth performance, and our results reflect this.}
\label{tab:abl1_old}

\end{table*}
















==> ablation/ablation2.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|c|c|c||c|c|c|c|}
\hline
 & \multicolumn{2}{c||}{Resolution (px/mm)} & \multicolumn{4}{c|}{Errors (depth weight inits)} \\ \hline
Fovea & Defocused & WAC & Focused & Defocused & WAC & Random \\ \hline \hline

1 & 31.30 (0.2) & 27.11 (0.75) &  &  &  &  \\ \hline
3 & 31.30 & 27.11 &  &  &  &  \\ \hline 
5 & 31.30 & 27.11 &  &  &  &  \\ \hline \hline
1 & 31.30 & 22.14 (0.5) &  &  &  &  \\ \hline
3 & 31.30 & 22.14 &  &  &  &  \\ \hline 
5 & 31.30 & 22.14 &  &  &  &  \\ \hline \hline
1 & 31.30 & 15.65 (0.25) &  &  &  &  \\ \hline
3 & 31.30 & 15.65 &  &  &  &  \\ \hline 
5 & 31.30 & 15.65 &  &  &  &  \\ \hline \hline \hline

1 & 15.65 (0.05) & 13.56 (0.75) & 5.382 & 5.544 & 5.621 &  \\ \hline
3 & 15.65 & 13.56 &  &  &  &  \\ \hline
5 & 15.65 & 13.56 &  &  &  &  \\ \hline \hline
1 & 15.65 & 11.07 (0.5) &  &  &  &  \\ \hline
3 & 15.65 & 11.07 &  &  &  &  \\ \hline
5 & 15.65 & 11.07 &  &  &  &  \\ \hline \hline
1 & 15.65 & 7.83 (0.25) &  &  &  &  \\ \hline
3 & 15.65 & 7.83 &  &  &  &  \\ \hline
5 & 15.65 & 7.83 &  &  &  &  \\ \hline \hline \hline

1 & 7.82 (0.0125) & 6.78 (0.75) &  &  &  &  \\ \hline
3 & 7.82 & 6.78 &  &  &  &  \\ \hline
5 & 7.82 & 6.78 &  &  &  &  \\ \hline \hline
1 & 7.82 & 5.53 (0.5) &  &  &  &  \\ \hline
3 & 7.82 & 5.53 &  &  &  &  \\ \hline
5 & 7.82 & 5.53 &  &  &  &  \\ \hline \hline
1 & 7.82 & 3.9 (0.25) &  &  &  &  \\ \hline
3 & 7.82 & 3.9 &  &  &  &  \\ \hline
5 & 7.82 & 3.9 &  &  &  &  \\ \hline 
\end{tabular}
\caption{Altering number of fovea, defocused and wac resolutions, with different depth weight initialization. Numbers in parenthesis are sanity checks, they are actual parameters used in image formation model, will delete.}
\label{tab:abl2}
\end{table*}

==> ablation/att.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFCE93}\textbf{Error (RMSE)}} \\ \cline{6-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{\begin{tabular}[c]{@{}c@{}}Focused \\ Epoch Init\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{\begin{tabular}[c]{@{}c@{}}Epochs \\ (FT/Total)\end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Depth Step (Decay Epoch)}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Attention Step (Decay Epoch)}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Sep Weight}} & \cellcolor[HTML]{FFCE93}\textbf{Learned} & \cellcolor[HTML]{FFCE93}\textbf{Random} \\ \hline
None & 20/20 & 1e-4 (15) & 1e-4 (15) & 1e-4 & 5.199 & 5.208 \\ \hline
10 & 20/30 & 1e-6 (5) & 1e-4 (15) & 1e-4 & 5.088 & 5.147 \\ \hline
10 & 20/30 & 1e-6 (5) & 1e-4 (15) & 1e-3 & 5.105 & 5.140 \\ \hline
20 & 20/30 & 1e-6 (5) & 1e-4 (15) & 1e-4 & 5.109 & 5.170 \\ \hline \hline

F 10 &  & 1e-6 (10) & 1e-4 (15) & 1e-4 &  &  \\ \hline 
E 10 &  & 1e-5 (5) & 1e-4 (15) & 1e-4 &  &  \\ \hline 
G 10 &  & 1e-5 (10) & 1e-4 (15) & 1e-4 &  &  \\ \hline 
H 10 &  & 1e-5 (10) & 1e-4 (10) & 1e-4 &  &  \\ \hline 

\end{tabular}}
\caption{Experiments for first row of Table 1. Once optimal numbers found for row 1, will repeat for all resolutions. Random errors involve using the new depth weights but with random attention.}
\label{tab:att_tab}
\end{table*}

==> ablation/oracle_table.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{ECF4FF} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFCCC9}Bandwidth (px/mm)} & \multicolumn{7}{c|}{\cellcolor[HTML]{ECF4FF}Errors (RMSE)} \\ \hline
\rowcolor[HTML]{ECF4FF} 
\cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{ECF4FF} & \multicolumn{2}{c|}{\cellcolor[HTML]{ECF4FF}Target Res} & \multicolumn{2}{c|}{\cellcolor[HTML]{ECF4FF}Low-res WAC} & \cellcolor[HTML]{ECF4FF} & \cellcolor[HTML]{ECF4FF} \\ \cline{5-8}
\rowcolor[HTML]{ECF4FF} 
\multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}Full Resolution} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}Target Resolution} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}Low-res WAC} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}Full Res} & 20 epochs & Finetune & 20 epochs & Finetune & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}\textbf{\begin{tabular}[c]{@{}c@{}}Hand design \\ \end{tabular}}} & \multirow{-2}{*}{\cellcolor[HTML]{ECF4FF}\textbf{\begin{tabular}[c]{@{}c@{}} Oracle (ground-truth SaccadeCam) \\  \end{tabular}}} \\ \hline
70 & 31.30 & 27.11 & 4.960 & 5.188 & 5.089 & 5.238 & 5.136 & 5.112 &  \textbf{4.850} \\ \hline
70 & 31.30 & 22.14 & 4.960 & 5.188 & 5.089 & 5.275 & 5.180 & 5.163 &  \textbf{4.846} \\ \hline
70 & 31.30 & 15.65 & 4.960 & 5.188 & 5.089 & 5.507 & 5.311 & 5.282 &  \textbf{4.848} \\ %\hline
%70 & 7.82 & 6.78 & 4.960 & 7.378 & 6.454 & 8.317 & 6.688 & \textbf{7.308} & \multicolumn{1}{l|}{} \\ %\hline
%70 & 7.82 & 5.53 & 4.960 & 7.378 & 6.454 & 9.382 & 7.155 & \textbf{7.341} & \multicolumn{1}{l|}{} \\ %\hline
%70 & 7.82 & 3.90 & 4.960 & 7.378 & 6.454 & 11.875 & 7.786 & 8.327 & \multicolumn{1}{l|}{} \\ 
\hline
\end{tabular}}
\caption{We motivate our method with a compelling example from the KITTI dataset \cite{geiger2013vision}. We compare a full resolution of $70$ px/mm (conventional KITTI imagery) with a target resolution of $31.30$ px/mm. As expected, full resolution does far better than both target resolution and a low-res image (which we call the wide angle camera or WAC). In the last column, we compute an ``Oracle" SaccadeCam by using ground-truth LIDAR to find the places where WAC might benefit from higher resolution, and replacing these with full resolution monocular depth. The results show that the Oracle beats both target and full resolution, showing that \emph{distributing resolution} adaptively can provide the best depth. Oracle SaccadeCam even beats a hand-designed attention mask, created by selecting the regions where full resolution outperforms the low-res WAC images. In Sect. \ref{sec:algo} we describe our algorithms to extract this potential of SaccadeCam. 
}
\label{tab:oracle_old}
\end{table*}

==> ablation/random.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{FFCE93} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{FFCCC9}\textbf{Resolution (px/mm)}} & \multicolumn{7}{c|}{\cellcolor[HTML]{FFCE93}\textbf{Errors (RMSE)}} \\ \hline
\rowcolor[HTML]{FFCE93} 
\cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCCC9} & \cellcolor[HTML]{FFCE93} & \cellcolor[HTML]{FFCE93} & \cellcolor[HTML]{FFCE93} & \cellcolor[HTML]{FFCE93} & \multicolumn{3}{c|}{\cellcolor[HTML]{FFCE93}\textbf{Random}} \\ \cline{8-10} 
\rowcolor[HTML]{FFCE93} 
\multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Focused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{Defocused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCCC9}\textbf{WAC}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCE93}\textbf{Focused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCE93}\textbf{Defocused}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCE93}\textbf{WAC}} & \multirow{-2}{*}{\cellcolor[HTML]{FFCE93}\textbf{Oracle}} & \textbf{1} & \textbf{3} & \textbf{5} \\ \hline
70 & 31.30 & 27.11 & 4.960 & 5.188 & 5.238 & 4.850 & 5.102 &  & 5.094 \\ \hline
70 & 31.30 & 22.14 & 4.960 & 5.188 & 5.275 & 4.846 & 5.119 &  & 5.125 \\ \hline
70 & 31.30 & 15.65 & 4.960 & 5.188 & 5.507 & 4.848 & 5.226 &  & 5.189 \\ \hline
70 & 15.65 & 13.56 & 4.960 & 5.426 & 5.681 & 5.123 & 5.404 &  & 5.402 \\ \hline
70 & 15.65 & 11.07 & 4.960 & 5.426 & 6.082 & 5.052 & 5.541 &  & 5.532 \\ \hline
70 & 15.65 & 7.83 & 4.960 & 5.426 & 7.743 & 5.236 & 5.989 &  & 5.917 \\ \hline
70 & 7.82 & 6.78 & 4.960 & 7.378 & 8.317 & 7.308 & 6.502 &  & 6.416 \\ \hline
70 & 7.82 & 5.53 & 4.960 & 7.378 & 9.382 & 7.341 & 6.636 &  & 6.623 \\ \hline
70 & 7.82 & 3.90 & 4.960 & 7.378 & 11.875 & 8.327 & 7.049 &  & 6.908 \\ \hline
\end{tabular}}
\caption{Random is initialized with 10 epoch focused weights (focused trained for 20 epochs) and finetuned for 3 epochs. The finetuned equiangular networks are initialized with 10 epoch focused weights and finetuned for 3 epochs just as random.}
\label{tab:random}
\end{table*}

==> sections/teaser.tex <==
\newcommand*{\vsepfbox}[1]{%
  \begingroup
    \sbox0{\fbox{#1}}%
    \setlength{\fboxrule}{0pt}%
    \mbox{\kern-\fboxsep\fbox{\unhbox0}\kern-\fboxsep}%
  \endgroup
}

\setlength\fboxrule{1pt}

\newcommand{\lmrgn}{-1.8mm}

%\newcommand{\scl}{0.072}
\newcommand{\scl}{0.105}

\vspace{-8mm}

% \begin{center}
%\vsepfbox{
\begin{varwidth}{\textwidth} \centering 
\hspace{\lmrgn} 
\includegraphics[width=\textwidth]{LaTeX/figs/teaser.png}
\end{varwidth}
\captionof{figure}{SaccadeCam: Given limited bandwidth, we adaptively distribute resolution onto regions of interest (fovea) as well as onto a low resolution wide-angle image. In (a) we show the low-res image, and we in (b) train a self-supervised network to produce attention masks. The remaining bandwidth is allocated onto fovea using this attention mask, rendering a monocular \emph{SaccadeCam} image (c) from which depth estimation can occur (d). In Table \ref{tab:abl1} and Fig. \ref{fig:results}, we show how SaccadeCam provides superior depth results to the conventional, uniformly distributed bandwidth.\\}
\label{fig:teaser}

%\end{center}
